Ownership in low-level intermediate representation

The concept of ownership in high level languages can aid both the programmer and the compiler to reason about the validity of memory operations. Previously, ownership semantics has been used successfully in high level automatic program verification to model a reference to data by a first order logic (FOL) representation of data instead of maintaining an address map. However, ownership semantics is not used in low level program verification. We have identified two challenges. First, ownership information is lost when a program is compiled to a low level intermediate representation (e.g., in LLVM IR). Second, pointers in low level programs point to bytes using an address map (e.g., in unsafe Rust) and thus the verification condition (VC) cannot always replace a pointer by its FOL abstraction. To remedy the situation, we develop ownership semantics for an LLVM like low level intermediate representation. Using these semantics, the VC can opportunistically model some memory accesses by a direct access of a pointer cache that stores byte representation of data. This scheme reduces instances where an address map must be maintained, especially for mostly safe programs that follow ownership semantics. For unsafe functionality, memory accesses are modelled by operations on an address map and we provide mechanisms to keep the address map and pointer cache in sync. We implement these semantics in SEABMC, a bit precise bounded model checker for LLVM. For evaluation, the source programs are assumed to be written in C. Since C does not have ownership built in, suitable macros are added that introduce and preserve ownership during translation to LLVM like IR for verification. This approach is evaluated on mature open source C code. For both handcrafted benchmarks and practical programs, we observe a speedup of $1.3x-5x$ during SMT solving.

==> assets/opsem/borrow.tex <==
% borrow.tex
\begin{tabular}{|c|c|c|c}
\hline
Register & U & RC & Ret_U \\
\hline
P & \logsym{1} & \logsym{1} & \logsym{\(\mu\)} \\
\hline
\end{tabular}

% TikZ picture for the arrow
\begin{tikzpicture}[remember picture, overlay]
\node (first) at (0,-0.25) {};
\node (second) at (2.7, -0.25) {};
\draw[thick, -latex] (first) -- (second);
\end{tikzpicture}

\vspace{2ex} % Space between tables

\( S, B = \text{borrow}\ P\)

\vspace{2ex} % Space between tables

\begin{tabular}{|c|c|c|c}
\hline
Register & U & RC & Ret_U \\
\hline
B & \logsym{1} & \logsym{1} & \logsym[orange]{x} \\
\hline
S & \logsym[orange]{x} & \logsym{1} & \logsym{\(\mu\)} \\
\hline
\end{tabular}


==> assets/opsem/borrow_check.tex <==
% borrow.tex
\begin{tabular}{|c|c|c|c}
\hline
Register & U & RC & Ret_U \\
\hline
P & \logsym{1} & \logsym{1} & \logsym{\(\mu\)} \\
\hline
\end{tabular}

% TikZ picture for the arrow
\begin{tikzpicture}[remember picture, overlay]
\node (first) at (0,-0.25) {};
\node (second) at (2.7, -0.25) {};
\draw[thick, -latex] (first) -- (second);
\end{tikzpicture}

\vspace{2ex} % Space between tables

\( S, B = \text{borrow}\ P\)

\vspace{2ex} % Space between tables

\begin{tabular}{|c|c|c|c}
\hline
Register & U & RC & Ret_U \\
\hline
B & \logsym{1} & \logsym{1} & \logsym[orange]{x} \\
\hline
S & \logsym[orange]{x} & \logsym{1} & \logsym{\(\mu\)} \\
\hline
\end{tabular}


==> background.tex <==
\section{Background}
\label{sec:background}
We present background on low level syntax and semantics for \seair, an enhanced version of \llvm IR that executes in the \seabmc model checking engine.
We then look at the VCGen process.
The section ends with a high level modelling of safe \rust for verification using prophecy variables.

\subsection{\seabmc and \seair}
\label{sec:seabmc-background}
We now present the \seair language and its semantics.

\bparagraph{\seabmc}
\seabmc is a bit-precise bounded model engine for \seahorn.
It generates verification conditions (VCGen) for a program in \llvm bitcode format in \smt format.
A high level program (in C or \rust) is translated to \llvm bitcode and extended with explicit dependency information between memory operations, which we call \seair.
In \seair, all memory operations are pure, i.e., there is no global memory, and no side-effects.
A \seair program then goes through a series of program transformations to for VCGen. Ultimately the program is reduced to a pure data-flow form in which all instructions execute in parallel, and is only then, converted to \smtlib supported logic.

To improve checking for safety properties, we attach additional information to pointers (so called \emph{fat}) and to memory (so called \emph{shadow}). This simplifies tracking of various program metadata for modelling safety properties. As an example, we can use fat pointers to check for out of bounds array access and shadow memory to check for immutability of read only memory. While existing tools report memory safety analysis, \seabmc can capture metadata of arbitrary size since we are not constrained by concrete pointer or memory width. Additionally, we model pointer provenance. This allows us to catch out-of-bounds accesses which might be missed by tools like \llbmc~\cite{DBLP:conf/vstte/MerzFS12} and \textsc{ASAN}~\cite{DBLP:conf/usenix/SerebryanyBPV12}.

\begin{figure}[t]
\centering
\begin{minipage}{0.9\linewidth}
\scriptsize
%\raggedleft
\begin{bnf*}
%\bnfprod{P}
%		{\bnfpn{F}} \\
\bnfprod{PR}
		{\texttt{fun main()}\bnfts{\{} \bnfpn{BB}^{\mathord+} \bnfts{\}}} \\
\bnfprod{BB}
        {\bnfpn{L}\bnfsp\texttt{:}\bnfsp \bnfpn{PHI} ^{\mathord*} \bnfsp \bnfpn{S}^+ \bnfsp (\bnfpn{BR}} \bnfor \texttt{halt})\\
\bnfprod{BR}
        {\texttt{br} \bnfsp \bnfpn{E},\ \bnfpn{L},\ \bnfpn{L} \bnfor \texttt{br} \bnfsp \bnfpn{L}} \\
\bnfprod{PHI}{
        \begin{bnfsplit}
        \bnfpn{R} = \texttt{phi} \bnfsp \texttt{[}\bnfpn{R},\ \bnfpn{L} \texttt{]} (\texttt{,[}\bnfpn{R},\ \bnfpn{L} \texttt{]})^* \bnfor \\
        \bnfpn{M} = \texttt{phi} \bnfsp \texttt{[}\bnfpn{M},\ \bnfpn{L}\texttt{]} (\texttt{,[}\bnfpn{M},\ \bnfpn{L}\texttt{]})^* \bnfor \\
        \bnfpn{P} = \texttt{phi} \bnfsp \texttt{[}\bnfpn{P},\ \bnfpn{L} \texttt{]} (\texttt{,[}\bnfpn{P},\ \bnfpn{L} \texttt{]})^*
        \end{bnfsplit}
        } \\
\bnfprod{S}
        {\bnfpn{RDEF} \bnfor \bnfpn{MDEF} \bnfor \bnfpn{VS}} \\
\bnfprod{RDEF}{
      \begin{bnfsplit}
      \bnfpn{R} = \bnfpn{E} \bnfor
      \bnfpn{P},\ \bnfpn{M} = \texttt{alloca} \bnfsp \bnfpn{R},\ \bnfpn{M} \bnfor \\
      \bnfpn{P},\ \bnfpn{M} = \texttt{malloc} \bnfsp \bnfpn{R},\ \bnfpn{M} \bnfor
      \bnfpn{R} = \texttt{load} \bnfsp \bnfpn{P}, \bnfsp \bnfpn{M} \bnfor \\
      \bnfpn{P} = \texttt{load} \bnfsp \bnfpn{P}, \bnfsp \bnfpn{M} \bnfor
      \bnfpn{M} = \texttt{free} \bnfsp \bnfpn{P}, \bnfsp \bnfpn{M} \bnfor \\
      \bnfpn{R} = \texttt{isderef} \bnfsp \bnfpn{R}, \bnfsp \bnfpn{R} \bnfor
      \bnfpn{R} = \texttt{isalloc} \bnfsp \bnfpn{R}, \bnfpn{M} \bnfor
      \bnfpn{R} = \texttt{ismod} \bnfsp \bnfpn{R}, \bnfsp \bnfpn{M}
      \end{bnfsplit} }\\
\bnfprod{MDEF}
        {\bnfpn{M} = \texttt{store} \bnfsp \bnfpn{R}, \bnfsp \bnfpn{P}, \bnfsp \bnfpn{M} \bnfor
         \bnfpn{M} = \texttt{store} \bnfsp \bnfpn{P}, \bnfsp \bnfpn{P}, \bnfsp \bnfpn{M}} \\
\bnfprod{VS}
        {\texttt{assert} \bnfsp \bnfpn{R} \bnfor \texttt{assume} \bnfsp \bnfpn{R}} \\
\end{bnf*}
\end{minipage}%
%\vspace{-0.15in}
\caption{Simplified grammar of \seair, where \texttt{E}, \texttt{L} \texttt{R}, \texttt{P} and \texttt{M} are expressions, labels, scalar registers, pointer registers and memory registers, respectively.}
\label{fig:seair-syntax}
%\vspace{-0.2in}
\end{figure}

\begin{figure}[t]
  \begin{lstlisting}[language=C, escapechar=@]
extern void escapeToMemory(char *);
int main() {
  char *p = (char *)malloc(sizeof(char));
  char c = nd_char();
  assume (c == 0);
  *p = c;
  char *b = p;
  if (nd_bool()) {
    c = nd_char();
    assume(c > 1);
    *b = c;
    escapeToMemory(b);
  }
  sassert(*p == 0 || *p > 1);
  return 0;
}
\end{lstlisting}%
%\vspace{-0.3in}
\caption{An example C program.}
\label{fig:example-C}
%\vspace{-0.25in}
\end{figure}%


\newsavebox{\figrpd}
\begin{lrbox}{\figrpd}%
\begin{lstlisting}[numbers=none]
fun main() {
BB0:
  M2 = mem.init()
  P0, M0 = malloc 1, M2
  R0 = nd_char()
  R1 = R0 == 0
  R2 = nd_bool();
  R3 = R2 == 0
  br R3, ERR, BB1

BB1:
  R5 = nd_char()
  R6 = R5 > 1
  R7 = R1 && R6
  M1 = store R5, P0, M0
  escapeToMemory(P0)
  R8 = load P0, M1
  br ERR

ERR:
  R9 = select R3, R1, R7
  R10 = select R3, R0, R8
  R11 = R10 == 0
  R12 = R10 > 1
  R13 = R9 || R12
  R14 = not R13
  A = R9 && R14
  assume A
  assert false
  halt
}
\end{lstlisting}
\end{lrbox}%

\newsavebox{\figformula}
\begin{lrbox}{\figformula}%
$
\begin{array}{l}
\sind[1] p_{0}.\base = \mathit{addr}_{0} \land{} p_{0}.\off = 0 \land{} p_{0}.\sz = 1 \land{} \\
\sind[1] r_{1} = (r_{0} = 0) \land{} \\
\sind[1] r_{3} = (r_{2} = 0) \land{} \\
\sind[1] r_{6} = r_{5} > 1 \land{} \\
\sind[1] r_{7} = r_{1} \land{} r_{6} \land{} \\
\sind[1] m_{1} = \mathit{write}(m_{0}, r_{5}, p_{0}) \land{} \\
\sind[1] r_{8} = \mathit{read}(m_{1}, p_{0}) \land{} \\
\sind[1] r_{9} = \mathit{ite}(r_{3}, r_{1}, r_{7}) \land{} \\
\sind[1] r_{10} = \mathit{ite}(r_{3}, r_{0}, r_{8}) \land{} \\
\sind[1] r_{11} = r_{10} = 0 \land{} \\
\sind[1] r_{12} = r_{10} > 1 \land{} \\
\sind[1] r_{13} = (r_{9} \lor r_{12}) \land{} \\
\sind[1] r_{14} = \neg r_{13} \land{} \\
\sind[1] a = r_{9} \land{} r_{14} \land{} \\
\sind[1] a \land{} \\
\sind[1] \neg \mathit{false}
\end{array}
$
\end{lrbox}%
\begin{figure}[t]
%\begin{tabular}{l l}
\begin{subfigure}[t]{0.4\textwidth}
\scalebox{1}{\usebox{\figrpd}}
\caption{Pure-Dataflow (PD)}
\label{fig:reducedPD}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
\raisebox{1.7cm}{\scalebox{0.8}{\usebox{\figformula}}}
\caption{\smtlib}
\label{fig:vc-code}
\end{subfigure}
%\end{tabular}
%\vspace{-0.1in}
\caption{Program from Fig.~\ref{fig:example-C} in PD and \smtlib forms. Note that the \code{store} and \code{load} instructions generate $\mathit{write}$ and $\mathit{read}$ expressions.}
\label{fig:code-vc-translate}
%\vspace{-0.3in}
\end{figure}

\bparagraph{The \seair language.}
\cref{fig:seair-syntax} shows the simplified syntax of \seair, which is the source language for VCGen.
Here, we present a simplified version
with many features removed, e.g., types, expressions, function calls, etc.
However, we assume that the type of each register is known (but not shown).
We use \code{R} to represent a scalar register, \code{P} for a pointer register and \code{M} for a memory register.
A legal \seair program is assumed to be in a Static Single Assignment
(SSA) form with all registers are assigned before use, all expressions well-typed and a program
always ending with a \tcode{halt}.

\subsection{VCGen.}

A high-level program,for example in C, is translated to \seair.
\seahorn then transforms the \seair in a pure data-flow form that is used for generating VCs.
In reduced PD form, all control dependence has been replaced by data dependence and the program is in a single basic block.

We explain the pipeline with a simple C program shown in~\cref{fig:example-C}.
The program allocates memory dynamically with address in \code{p}.
A non-deterministic character (returned by \code{nd_char()}) is written to \code{p}'s address.
The program then creates an alias \code{b} to \code{p}.
It then conditionally constraints the non-deterministic character, through \code{b} and finally asserts the range of the character using \code{p}.
The property being checked is valid so the assertion passes.
The \seair version in reduced PD form is in \cref{fig:reducedPD}.
The corresponding VC is in \cref{fig:vc-code}.
The VC is a \smtlib program.
For simplicity of presentation, we assume that two fundamental sorts are used in
the encoding: bit-vector of $64$ bits, \bv{64}, and a map between bit-vectors, $\bv{64} \to
\bv{64}$.\footnote{In practice, \seabmc supports multiple
  bit-widths for scalars, and different ranges for values for maps.}

In addition, we use the following helper sorts:
$\scalar:\bv{64},$
$\ptrsort: \langle \scalar_{1}, \dots, \scalar_{m} \rangle,$
$\memsort: \langle (\bv{64} \to \bv{64})_{1}, \dots, (\bv{64} \to \bv{64})_{n} \rangle \textit{ where } n \geq m$
Here \scalar is sorts of scalars, \ptrsort of
pointers, and \memsort of memories.

The \ptrsort is a composite type on account of metadata that we want to carry at a fat pointer.
For example, a fat pointer carries the following allocation information:
\begin{itemize}
  \item [$\base$] to store the allocation start address of a pointer,
  \item [$\off$] to store the offset of the current pointer, and,
  \item [$\sz$] to store the size of the allocation.
\end{itemize}
Similarly, \memsort is also a composite type and be wide enough to store a fat pointer and may also carry additional shadow program state tied to a memory location.
%We describe more details about fat pointers and shadow memory in~\cref{sec:lang} and~\cref{sec:prop} respectively.

% We now turn our attention to the translation function $\symfun$ that encodes a \seair
% program into a VC.
% $\symfun$ is defined recursively,
% bottom up, on the abstract syntax tree of \seair. First, each register,
% \code{R}, is mapped to a symbolic constant $\sym{\text{\code{R}}}$ of an
% appropriate sort. To simplify the
% presentation, we use a lower-case math font for constants corresponding to the register. For example, in \cref{fig:reducedPD},
% $\sym{\tcode{R0}}$ is $r_0$ of \scalar sort,
% $\sym{\tcode{P0}}$ is $p_0$ of \ptrsort sort, and
% $\sym{\tcode{M0}}$ is $m_0$ of \memsort sort,
% respectively.

% Second, each expression \code{E} in \seair is mapped into a corresponding
% \smtlib expression $\sym{\tcode{E}}$. We omit the details of this step since they are
% fairly standard. For example, a \code{select} is translated into an
% $\mathit{ite}$, scalar comparision, such as \code{R0 > 1} is translated into
% bit-vector comparision \code{bvsgt}, etc.

% Finally, $\symfun$ translates each statement into an equality. For example, \code{R = E} is translated into $r=e$, where $e$ is $\sym{\tcode{E}}$. For example, in \cref{fig:reducedPD}, \code{R12 = select R9,R11,R7} is translated into $a = \mathit{ite}(r_9, r_{11}, r_7)$ in \cref{fig:vc-code}.

% Translating \code{alloca} and \code{malloc} requires a memory allocator.
% We parameterize $\symfun$ by an allocation function $\falloc: A \to
% \ptrsort$ that maps allocation expressions in $A$ to values of pointer
% sort. For example, in \cref{fig:vcg}, \code{P1, M1 = alloca R0, M0} is translated
% into $p_1 = \falloc(\tcode{alloca} ~ \tcode{R0} ~ \tcode{M0}) ~ \land ~ m_1 =
% m_0$, and is reduced to $p_1 = \mathit{addr}_0 \land m_1 = m_0$, where
% $\mathit{addr}_0$ is the return value of $\falloc$.

% Note that \cref{fig:vc-code} shows generated $\mathit{read}$ and $\mathit{write}$ expressions.
% These expressions wrap a choice between low-level address space based memory representations.
% \seabmc currently offers two options -- \textit{Arrays} and $\lambda$--\textit{abstractions} as shown in~\cref{fig:read-write}.
% In this paper, we show cases when ownership semantics can help minimize occurrence of $\mathit{read}$ and $\mathit{write}$ expressions in the final \smt program that is sent to a solver.

% \begin{figure}[t]
% \small
% \[
% \begin{lgathered}
% \small
% \scalebox{0.9}{$  \begin{aligned}
% \sym{\tcode{R = E}}  &\sdef  r = e &
% \sym{\tcode{assume R}}  &\sdef  r &
% \sym{\tcode{assert R}}  &\sdef  \neg r
% \end{aligned}$}\\
% \scalebox{0.9}{$ \begin{aligned}
% \sym{\tcode{M1 = store R1,P2,M0}} & \sdef m_1 = \mathit{write}(m_0, r_1, p_2) \\
% \sym{\tcode{R1 = load P0,M}} & \sdef p_1 = \mathit{read}(m, p_0) \\
% \end{aligned} $}\\
% \scalebox{0.9}{$ \begin{multlined}
% \sym{\tcode{P1,M1 = alloca R0,M0}}  \sdef p_1 = \falloc(\tcode{alloca R0,M0}) ~\land~ m_1 = m_0
% \end{multlined} $}\\
% \scalebox{0.9}{$\begin{multlined}
% \sym{\tcode{P1,M1 = malloc R0,M0}} \sdef p_1 =
%                                               \falloc(\tcode{malloc R0,M0})  ~\land~ m_1 = m_0
% \end{multlined}$}
% \end{lgathered}
% \]
% %\vspace{-0.1in}
% \caption{Definition of $\symfun$.}
% \label{fig:vcg}
% %\vspace{-0.3in}
% \end{figure}


% \begin{figure}[t]
% {\footnotesize
% \[
% \begin{array}{r| l l}
% & \tcode{Array} & \lambda \\
% \hline
% \mathit{read}(m, p_0) & \tcode{select}~ m ~ p_0 ~ & m(p_0)\\
% \mathit{write}(m_0, r_1, p_2) & \tcode{store}~ m_0 ~ r_1 ~ p_2 & \lambda x. \mathit{ite}(x = p_2, r_1, m_0(x))\\
% \end{array}
% \]
% }
% %\vspace{-0.1in}
% \caption{Translation of \textit{read} and \textit{write}.}
% \label{fig:read-write}
% %\vspace{-0.2in}
% \end{figure}

% \bparagraph{Fat pointers and Shadow Memory.}
% Intuitively, we want to represent each fat pointer as a tuple of values that
% collectively represent the value of the pointer and all the metadata (i.e., \emph{fat}) that is attached to it. We do not put restrictions on the number of values nor their sorts.
% However, we assume that there is a function $addr$ that maps a pointer to an
% expression representing an address. Thus, for a pointer register \rP,
% \sym{\tcode{P}} is a tuple $ \langle t_{1}, \ldots, t_j \rangle $ of $j$
% constants that represents the pointer, and $addr (\langle t_{1}, \ldots, t_j
% \rangle) $ is an address of that pointer. For example, a common case is to use
% the first element of the tuple to represent the address: $addr(\langle t_1,
% \ldots, t_j \rangle) = t_1$.

% Formally, we re-define \ptrsort to be a tuple of sorts, written as $ \langle
% s_{1}, \ldots, s_{j} \rangle $. We say that a tuple $\tau = \langle c_{1},
% \ldots, c_{p} \rangle $ of $p$ constants is of a tuple sort $ \langle s_{1},
% \ldots, s_{p} \rangle$ iff, for each $0 < i \leq p$, $c_i$ is of sort $s_i$.
% Tuples of sorts, and tuples of constants are only present during VCGen, but not
% in the final verification condition. For that, we rewrite equality between two
% tuples as conjunction of equalities between their elements, and use $\tau.i$
% for the $i$th element of tuple $\tau$.

% Similarly, we re-define \memsort for a memory register
% \code{M} to be a tuple of values that store the program and the shadow states. Thus, $\sym{\tcode{M}} = \langle v_{0}, \ldots, v_{k} \rangle $,
% where each $v_i$ is the sort $\mathit{bv}(64) \to \mathit{bv}(64)$. If a pointer
% is represented by a $j$-tuple, we assume that memory is represented by a
% $k$-tuple, with $k \geq j$, so that the first $j$ entries in a memory register
% are wide enough to store the fat pointer. Specifically, we require that
% the sort of $v_j$ is same as sort of $t_j$ for $1 \leq j \leq k$.

% % Pointer manipulating expressions, such as
% % pointer arithmetic (\code{gep}) and pointer-to-integer cast
% % (\code{ptoi}) are described
% % in~\cref{sec:ext}.

\subsection{Modeling borrows using prophecy variables.}

\begin{figure}[t]
  \centering
  \begin{lstlisting}[language=Rust]
    fn main() {
      let mut x = Box::new(10); // $x.\val=10$
      increment(&mut x); // $y.\val=x.\val \land{} x_{1}.\val=z \land{}  y.\ret{val}=x.\val$
      assert!(*x == 11); // $\neg (x_{1}.\val = 11)$
    }

    fn increment(b: &mut Box<i32>) { // $y.\val=b.\val \land{} y.\ret{val}=b.\ret{val}$
      **b += 1;  // $b_{1}.\val=b.\val+1 \land{} b_{1}.\ret{val}=b.\ret{val}$
    }  // $b_{1}.\ret{val} = b_{1}.\val$
  \end{lstlisting}
  \caption{A \rust program with a borrowed reference. The logical formulae (in comments) use prophecy variable $z$ to exchange data between owner $x$ and borrower $b$.}
  \label{fig:rust-prophecy-code}
\end{figure}

We motivate the carrying of a value at reference and prophecy variables through ~\cref{fig:rust-prophecy-code}.
Each line of code has a comment of a plausible VC generated by the associated computation.
The VC may be generated by a $sym$ function similar to one shown in~\cref{sec:seabmc-background}.
We imagine $x$ to be an \smt datatype with two arguments $\val$ and $\ret{val}$.
The $x.\val$ syntax selects the associated argument $\val$ from $x$.
In line 2, an initialization of a \code{Box} with $10$ does not induce a write to memory.
Instead, the value is \emph{carried} at the logical variable $x$ in $x.\val$.
In line 3, \code{x} is mutably borrowed by the function \code{increment}.
Here, the future value of $x$ is designated $x_{1}$.
$x_{1}.\val$ will only be known after \code{increment} returns.
We thus \emph{prophesize} that $x.\val$ will be a fresh non-deterministic variable $z$.
The borrowed reference variable is $y$.
We further \emph{entangle} $x_{1}.\val$ with $y.\ret{val}$ by equating them.
Now $x_{1}.\val$ will be whatever $y_{1}.\ret{val}$ is, and is $z$ in this line.

In the function \code{increment}, in line 7, the arguments of $y$ are equated to $b$.
Line 8 increments \code{b}.
The logical equivalent is now $b_{1}$.
$b_{1}.\val$ is set instead of updating memory.
In line 9, the function returns.
At this stage, $b_{1}.\ret{val}$ is constrained to be equal to $b_{1}.\val$
The prophecy is now complete.

In line 4, the \code{assert} again reads $x_{1}.\val$ instead of reading from memory and sees the value $11$.
Thus the VC correctly models the program by carrying values at references and thus avoiding a memory model with an address space.


==> intro.tex <==
\section{Introduction}
\label{sec:ownsem-intro}
Ownership of data in programs has been studied in a long line of academic research~\cite{DBLP:conf/pldi/FahndrichD02,DBLP:conf/pldi/GrossmanMJHWC02,DBLP:journals/toplas/MatsushitaTK21,DBLP:conf/ecoop/NobleVP98}.
More recently, the concept has gained attention due to \rust, a popular systems language that offers low level control like C/C++ and uses ownership semantics to record aliases and mutation of data.
Ownership semantics is specified by three rules~\cite{DBLP:journals/corr/abs-2011-06171}:
\begin{inparaenum}
  \item All values have exactly one owner;
  \item A reference to a value (borrow) cannot outlive the owner; and
  \item A value can have one mutable reference \emph{xor} many immutable references.
\end{inparaenum}

In verification of a system program, for example written in C/C++, the generated verification condition (VC) necessarily models memory accesses through an address space because a value (in memory) may have multiple mutable references.
There are different choices of address space based memory models that can be used but generally the VC becomes more complex.
In contrast, prior verification work on \rust programs has shown that the VC for a program that exclusively uses ownership semantics does not need to model an address space and removes the associated complexity.
This is because when references are unique, object data can be carried at the reference itself~\cite{DBLP:conf/tacas/DillGPQXZ22} without changing the meaning of the program and mutably borrowed aliases can exchange information using prophecy variables~\cite{DBLP:journals/toplas/MatsushitaTK21} or other means.

However, practical programs, including those written in \rust use \emph{mostly safe} accesses.
Most accesses occur through owning and borrowed pointers and are non--interleaving.
Some accesses our through raw pointers (in so-called \emph{unsafe} code-blocks) and may be interleaved.
Unsafe code is needed for expressivity, performance or for interacting with legacy code (e.g., written in C)~\cite{DBLP:journals/pacmpl/AstrauskasMP0S20}.
For example, in graph data structures multiple mutable aliases may refer to a single graph node for expressing the data structure correctly.
For verification, the introduction of unsafe code breaks the memory abstraction afforded by ownership semantics and \emph{prima facie} the VC now needs to, again, model memory accesses through an address space for the whole program.

This presentation explores a midway design point for VCGen of such programs.
This design offers opportunistic memory modelling in VCGen for whole program analysis where a program uses both ownership semantics (safe) and potentially interleaved (unsafe) accesses through raw pointers.
It allows for  the VC to be simplified by modelling memory accesses \emph{only} in the presence of mutable aliases and carry values of interest at a pointer, when the pointer follows ownership semantics.
Doing so, enables whole programs with ownership semantics to be verified in a scalable way.

The program can synchronize these values between pointer and memory at key points (safe--unsafe boundaries) in the program.
This scheme marries existing work in verification of high level safe Rust and unsafe C settings to allow efficient automatic verification of a wider class of programs.

Our scheme is operationalized in \seair, a low level language based on \llvm IR that executes on the \seabmc \bmc tool~\cite{DBLP:conf/fmcad/PriyaSBZVG22}.
We add ownership semantics for pointer creation and aliasing operations to \seair to create a new language \oseair.
We particularly use the low level \llvm IR language because:
\begin{inparaenum}
  \item all safe and unsafe operations are represented uniformly,
  \item the \rust compiler compiles to \llvm IR allowing future work to connect \rust to \oseair , and,
  \item it is straight-forward to generate VC from an \llvm program.
\end{inparaenum}
The \seabmc tool is thus enhanced to work with \oseair using fat pointers -- pointers that carry address information and additional metadata.
The data to be carried at a fat pointer has be scalar to keep the VC simple.
\sid{show a code example of how fat ptr vs shadow mem generate vc.}
We discuss this limitation and show that interesting typestate properties can be encoded as scalar data attached to pointers.
Finally, we provide an empirical evaluation \seabmc on \oseair programs compiled from \mbedtls open source project written in C.

% Additionally, we present (under-development):
% \begin{inparaenum}
%   \item a technique to check safety of an \oseair program under ownership semantics,
%   \item a discussion of what properties can be carried at references as values of interest,
%   \item an extensive evaluation of \seabmc on \oseair programs compiled from \mbedtls open source project written in C.
%  \end{inparaenum}
    

==> lang.tex <==
\section{VCGen with ownership semantics.}
\label{sec:lang}

Our goal is to carry a \voi at a fat pointer itself such that when the pointer is unique then all read and writes that touch this value can use a designated fat metadata slot without resorting to memory accesses in the \smt program.
The \voi itself can be a program value or program metadata that fits into a $\scalar$ datatype.
This is discussed more in~\cref{sec:prop}

To ascertain uniqueness of pointers, we present additional instructions (intrinsics) to \seair that introduce ownership, borrow and copy concepts to pointer operations.
These operations wrap existing pointer creation and aliasing operations (e.g., \code{gep}) with additional semantics so that a \voi carried with a unique pointer can be transferred between aliases if aliases do not interfere in read and writes (mutable borrow) or are read only (read only borrow).

We group the intrinsics into the following categories to ease presentation:
\begin{inparaenum}
	\item Creation and Properties,
	\item Mutable Borrow and Die,
	\item Read Only Borrow,
	\item Copy, and,
	\item Register--Memory transfer.
\end{inparaenum}
The syntax for ownership intrinsics in shown in~\cref{fig:own-syntax}.
Note that aliasing operations (mutable borrow, read only borrow and copy) consume the operand pointer and create a pair of result pointers.
In \oseair this creation of pairs is split across two operations -- e.g., mutable borrow is split into \mutborbor \code{p} that creates a \mutborptr\footnote{A portmanteau for mutably borrowed.} and \mutborsuc that creates a \sucptr .


% We first present the semantics of ownership operations in \oseair without the details of how a \voi is carried at a pointer. We then separately present how the \voi is retained and updated at a pointer itself.

% \bparagraph{Ownership Semantics.}
% In ownership semantics, pointers have additional meaning.
% These meanings are carried in new fat slots as shown in~\cref{tab:ownsem-fat-slots}.
% The intent of aliasing operations is motivated through pre-and-post conditions predicates that must hold before and after an operation as shown in~\cref{tab:ownsem-pre-post}.
% For example, a pointer becomes an \ownptr by going through an \mkown operation that consumes the original pointer. This \ownptr is the only alias (unique) and has read-write access.

% A mutable borrow operation creates a \mutborptr and a \sucptr.
% In a valid program, the \sucptr gets read-write access only after the \mutborptr has completed all reads and writes through it (i.e., has \emph{died}).
% A program explicitly marks death of a pointer using a \code{die} operation.
% Note that this scheme disallows interleaved accesses between \mutborptr and \sucptr.
% Also note that~\cref{tab:ownsem-pre-post} captures the final post-condition of a pointer.
% Therefore the \sucptr (S) post-condition ($s.\wok \land{} s.\rok \land s.\uc$) is only true after the \mutborptr dies. The in-between state of S is not captured by these semantics.
%Refining this scheme is \wip and we present next steps in~\cref{sec:safety}.

% A read only borrow operation creates a \roborptr and a \sucptr.
% Both pointers get interleaved, but read only, access until \roborptr dies.
% After this, the \sucptr gets read-write access.
% A copy operation creates two copying pointers\footnote{These are called raw pointers in \rust.}.
% Each \cpyptr has read write access.

% \bparagraph{}
Before considering the intrinsics, we first explain some helper macros in~\cref{fig:own_sem_helpers}.
The $\copyallocinfo$ macro equates allocation data between two fat pointers.
This follows the presentation from~\cref{sec:background}.
The $\entangle$ macro equates two \scalar symbols (e.g., $r_{1},r_{2}$ to an existentially quantified prophecy variable $x$. This is skolemized to a fresh non-deterministic variable.
When either $r_{1}$ or $r_{2}$ is constrained (by an assumption), the other symbol also sees the constraint.
This entanglement is key to modelling borrows.
Fat pointers contain a slot $\val$ for carrying a \voi.
They also contain a slot $\ret{val}$ that is meaningful for \mutborptr as a means to transfer a \voi to the \ownptr.
The $\copyvalinfo$ macro equates the value fields between two fat pointers.
The $\freshenval$ macro overwrites the $\val$ and $\ret{val}$ fat slots with fresh nondeterministic variables.
We now explain each category of ownership intrinsics.




\begin{figure}[t]
	\centering
	\begin{minipage}{0.9\linewidth}
		\scriptsize
		%\raggedleft
		\begin{bnf*}
			\bnfprod{S}
			{\dots \bnfor \bnfpn{OS}} \\
			\bnfprod{RDEF}{
				\begin{bnfsplit}
					\dots
					\bnfor \\
					\bnfpn{P} = \texttt{mk\_own} \bnfsp \bnfpn{P}
					\bnfor
					\bnfpn{P} = \texttt{begin\_unique} \bnfsp \bnfpn{P}
					\bnfor
					\bnfpn{P} = \texttt{end\_unique} \bnfsp \bnfpn{P}
					\bnfor \\
					\bnfpn{P} = \texttt{mut\_mkbor} \bnfsp \bnfpn{P}
					\bnfor
					\bnfpn{P} = \texttt{mut\_mkbor\_off} \bnfsp \bnfpn{P},\ \bnfsp \bnfpn{R}
					\bnfor
					\bnfpn{P} = \texttt{mut\_mksuc} \bnfsp \bnfpn{P}
					\bnfor \\
					\bnfpn{P} = \texttt{ro\_mkbor} \bnfsp \bnfpn{P}
					\bnfor
					\bnfpn{P} = \texttt{ro\_mkbor\_off} \bnfsp \bnfpn{P},\ \bnfsp \bnfpn{R}
					\bnfor
					\bnfpn{P} = \texttt{ro\_mksuc} \bnfsp \bnfpn{P}
					\bnfor \\
					\bnfpn{P} = \texttt{cpy\_mkcpy1} \bnfsp \bnfpn{P}
					\bnfor
					\bnfpn{P} = \texttt{cpy\_mkcpy1\_off} \bnfsp \bnfpn{P},\ \bnfsp \bnfpn{R}
					\bnfor
					\bnfpn{P} = \texttt{cpy\_mkcpy2} \bnfsp \bnfpn{P}
					\bnfor \\
					\bnfpn{P} = \texttt{set\_prop} \bnfsp \bnfpn{P}, \bnfsp \bnfpn{R}
					\bnfor
					\bnfpn{R} = \texttt{get\_prop} \bnfsp \bnfpn{P}
					\\
				\end{bnfsplit} }\\
			\bnfprod{MDEF}
			{\dots \bnfor
				\bnfpn{P},\ \bnfpn{M} = \texttt{mut\_mkbor\_mem2reg} \bnfsp \bnfpn{P},\ \bnfsp \bnfpn{M} \bnfor \bnfpn{M} = \texttt{mov\_reg2mem} \bnfsp \bnfpn{P}, \bnfsp \bnfpn{P}, \bnfsp \bnfpn{M}} \\
			\bnfprod{OS}
			{\texttt{die} \bnfsp \bnfpn{P}}
		\end{bnf*}
	\end{minipage}
	%\vspace{-0.15in}
	\caption{Grammar of new ownership semantics in \seair (now called \oseair), where \texttt{R}, \texttt{P} and \texttt{M} are scalar registers, pointer registers and memory registers, respectively.}
	\label{fig:own-syntax}
	%\vspace{-0.2in}
\end{figure}

% \newsavebox{\borrowcheckopsembox}
% \begin{lrbox}{\borrowcheckopsembox}
%   \input{assets/opsem/borrow_check.tex}
% \end{lrbox}

% \begin{figure}[htbp]
%   \centering
%   \usebox{\usebox{\borrowcheckopsembox}}
%   \caption{Operational semantics for checking borrow.}
%   \label{fig:borrow_check_opsem}
% \end{figure}


% \begin{table}[t]
% 	\centering
% 	\rowcolors{2}{purple!30}{pink!60}
% 	\begin{tabular}{|c|c|}
% 		\hline
% 		\rowcolor{gray!15}
% 		Fat slot & description                                                     \\
% 	$\own \colon boolean$       & \Ownptr: $true$ means pointer is owning.            \\
% 		$\uc \colon boolean$       & Unique count: $true$ means pointer is unique.            \\
% 		$\wok \colon boolean$      & Write ok: $true$ means write allowed through pointer.       \\
% 		$\rok \colon boolean$      & Read ok: $true$ means read allowed through pointer.         \\
% 		\hline
% 	\end{tabular}
% 	\label{tab:ownsem-fat-slots}
% 	\caption{Fat slots for ownership semantics (\ownsem slots).}
% \end{table}

% \begin{table}[t]
% 	\centering
% 	\rowcolors{2}{blue!40}{blue!15}
% 	\begin{tabular}{|c|c|p{35mm}|p{50mm}|}
% 		\hline
% 		\rowcolor{gray!15}
% 		row & Operation & Pre-condition & Final post-condition \\
%         1 & \code{b=mut_mkbor p,\ s=mut_mksuc p} &
%                                           $p.\uc \land{} p.\wok \land{} p.\rok$ &
%     $ \neg b.\own \land{} b.\uc \land{} b.\wok \land{} b.\rok \land{} s.\own=p.\own \land{} s.\uc \land{} s.\wok \land{} s.\rok$\\
% 		2 & \code{b=ro_mkbor p,\ s=ro_mksuc p} & $ite(p.\uc, p.\rok \land{} p.\wok, p.\rok \land \neg p.\wok)$ & $\neg b.\own \land{} b.\uc \land{} \neg b.\wok \land{} b.\rok \land{} s.\own=p.\own \land{} s.\uc \land{} s.\wok \land{} s.\rok$\\
% 		3 &	\code{c1=cpy_mkcpy1 p,\ c2=cpy_mkcpy2 p} &  $p.\wok \land{} p.\rok$ & $ \neg c_{1}.\own \land{}\neg c_{1}.\uc \land{} c_{1}.\wok \land{} c_{1}.\rok \land{} c_{2}.\own=p.\own \land{} c_{2}.\uc=p.\uc \land{} c_{2}.\wok \land{} c_{2}.\rok$\\
% 	  4 & \code{b,m1=mut_mkbor_mem2reg p,\ m0} &  $\exists b_{l} \cdot (b_{l}=read(m_{0},p) \land{} b_{l}.\own \land{} b_{l}.\wok \land{} b_{l}.\uc \land{} b_{l}.\rok)$ & $\neg b.\own \land{} b.\uc \land{} b.\wok \land{} b.\rok \land{} \exists p_{s} \cdot (p_{s}=read(m_{1},p) \land{} p_{s}.\own \land{} p_{s}.\wok \land{} p_{s}.\uc \land{} p_{s}.\rok)$ \\
%     5 & \code{m1=mov_reg2mem p,\ pp,\ m0} &  $p.\own \land{} p.\uc \land{} p.\wok \land{} p.\rok$ & $\exists p_{s} \cdot (p_{s}=read(m_{1},pp) \land{} p_{s}.\own \land{} p_{s}.\wok \land{} p_{s}.\uc \land{} p_{s}.\rok)$ \\
%     6 & \code{p1=mk_own p0} & $true$ & $p.\own \land{} p.\uc \land{} p.\wok \land{} p.\rok$ \\
% 		\hline
% 	\end{tabular}
% 	\label{tab:ownsem-pre-post}
% 	\caption{Pre and final post conditions on \ownsem slots for aliasing and \code{mk_own} operations.}
% \end{table}

\begin{figure}[t]
	\begin{lstlisting}[language=C]
extern void escapeToMemory(char *);
int main() {
  char *p = (char *)malloc(sizeof(char));
  *@\marktext{SEA\_MKOWN(p);}@* *@\label{line:own-example-C-mkown} @*
  char c = nd_char();
  assume (c == 0);
  *@\marktext{SEA\_SET\_PROP(p, c);}@* *@\label{line:own-example-C-setprop} @*
  *p = c;
  char *b;
  *@\marktext{SEA\_BORROW(b, p);}@*
  if (nd_bool()) {
    c = nd_char();
    assume(c > 1);
    *@\marktext{SEA\_SET\_PROP(b, c);}@*
    *b = c;
    escapeToMemory(b);
  }
  *@\marktext{SEA\_DIE(b);}@*
  char r;
  *@\marktext{SEA\_GET\_PROP(p, r);}@*
  sassert(r == 0 || r > 1);
  *@\marktext{SEA\_DIE(p);}@*
  return 0;
}
\end{lstlisting}%
	%\vspace{-0.3in}
	\caption{An example C program with ownership intrinsics wrapped in C Macros, highlighted in \marktext{yellow}.}
	\label{fig:own-example-C}
	%\vspace{-0.25in}
\end{figure}%


\newsavebox{\figownrpd}
\begin{lrbox}{\figownrpd}%
	\begin{lstlisting}
fun main() {
BB0:
  M3 = mem.init()
  P0, M0 = malloc 1, M3
  *@\marktext{P2 = mk\_own P0}@*
  R5 = nd_char()
  R6 = R5 == 0
  *@\marktext{P3 = set\_prop P2 R5}@*
  M1 = store R5, P3, M0
  *@\marktext{P5 = mut\_mkbor P3}@*
  *@\marktext{P6 = mut\_mksuc P3}@*
  R15 = nd_bool();
  R17 = R15 == 0
  br R17, ERR, BB1

BB1:
  R18 = nd_char()
  R19 = R18 > 1
  R20 = R6 && R19
  *@\marktext{P23 = set\_prop P5 R18}@*
  M2 = store R18, P23, M1
  escapeToMemory(P0)
  br ERR

ERR:
  R22 = select R17, R6, R20
  P24 = select R17, P5, P23
  *@\marktext{die P24}@*
  *@\marktext{R29 = get\_prop P6}@*
  R30 = R29 == 0
  R31 = R29 > 1
  R32 = R30 || R31
  A = not R32
  assume A
  assert false
  halt
}
\end{lstlisting}
\end{lrbox}%

\newsavebox{\figownformula}
\begin{lrbox}{\figownformula}%
	$
		\begin{array}{l}
			\sind[1] p_{0}.\base = \mathit{addr}_{0} \land{} p_{0}.\off = 0 \land{} p_{0}.\sz = 1 \land{}        \\
			\sind[1] \marktext{$p_{2} = \copyallocinfo(p_{2}, p_{0}) \land{} \freshenval(p_{2})$} \land{}        \\
			\sind[1] r_{6} = (r_{5} = 0) \land{}                                                                 \\
			\sind[1]\marktext{$ \copyallocinfo(p_{3}, p_{2}) \land{} p_{3}.\val = r_{5}$}  \land{}               \\
			\sind[1] \marktext{$\copyallocinfo(p_{5}, p_{3}) \land{} \copyallocinfo(p_{6}, p_{3}) \land{} $}     \\
			\sind[1] \marktext{$\entangle(p_{5}.\ret{val}, p_{6}.\val) \land{} p_{5}.\val = p_{3}.\val$} \land{} \\
			\sind[1] r_{17} = (r_{15} = 0) \land{}                                                               \\
			\sind[1] r_{19} = r_{18} > 1 \land{}                                                                 \\
			\sind[1] r_{20} = r_{6} \land{} r_{19} \land{}                                                       \\
			\sind[1] \marktext{$\copyallocinfo(p_{23}, p_{5}) \land{} p_{23}.\val = r_{18}$} \land{}             \\
			\sind[1] r_{22} = \mathit{ite}(r_{17}, r_{6}, r_{20}) \land{}                                        \\
			\sind[1] p_{24} = \mathit{ite}(r_{17}, p_{5}, p_{23}) \land{}                                        \\
			\sind[1] \marktext{$p_{24}.\ret{val} = p_{24}.val$} \land{} r_{22} \land{}                           \\
			\sind[1] \marktext{$r_{29} = p_{6}.\val$} \land{}                                                    \\
			\sind[1] r_{30} = r_{29} = 0 \land{}                                                                 \\
			\sind[1] r_{31} = r_{29} > 1 \land{}                                                                 \\
			\sind[1] r_{32} = (r_{30} \lor r_{31}) \land{}                                                       \\
			\sind[1] a = \neg r_{32} \land{}                                                                     \\
			\sind[1] a \land{}                                                                                   \\
			\sind[1] \neg \mathit{false}
		\end{array}
	$
\end{lrbox}%
\newsavebox{\figborrpd}
\begin{lrbox}{\figborrpd}%
	\begin{lstlisting}[numbers=none]
fun main() {
BB0:
  $\dots$
  P2 = mk_own P0
  *@
  \drawfatptr{p_2}{\val}{x}{\ret{\val}}{y}
  @*
  $\dots$
  p3 = set_prop P2 R5
  *@\drawfatptr{p_3}{\val}{r5}{\ret{\val}}{y}@*
  $\dots$
  P5 = mut_mkbor P3
  P6 = mut_mksuc P3
  *@
	\begin{tabular}{|c|c|c}
		\cellcolor{purple!30} $\mathit{ptr}$ & \cellcolor{purple!30} \val & \cellcolor{purple!30} \ret{\val} \\
		\cellcolor{pink!60} $\mathit{p5}$   & \cellcolor{pink!60} $\mathit{r_{5}}$   & \cellcolor{pink!60} $\boldsymbol{\mathit{z}}$ \\
    \cellcolor{orange!50} $\mathit{p6}$   & \cellcolor{orange!50} $\boldsymbol{\mathit{z}}$   & \cellcolor{orange!50} $\mathit{y}$
	\end{tabular}
  @*
  $\dots$
  br R17, ERR, BB1

BB1:
  $\dots$
  P23 = set_prop P5 R18
  *@\drawfatptr{p_{23}}{\val}{r_{18}}{\ret{\val}}{\boldsymbol{\mathit{z}}}@*
  $\dots$
  br ERR

ERR:
  $\dots$
  P24 = select R17, P5, P23
  *@\drawfatptr{p_{24}}{\val}{\mathit{ite}(r_{17}, r_5, r_{18})}{\ret{\val}}{\boldsymbol{\mathit{z}}}@*
  die P24
  *@\marktext[pink!60]{$\boldsymbol{\mathit{z}} = \mathit{ite}(r_{17}, r_5, r_{18})$}@*
  R29 = get_prop P6
  *@\marktext[pink!60]{$r_{29}=\boldsymbol{\mathit{z}}$}@*
  $\dots$
  halt
}
\end{lstlisting}
\end{lrbox}%

\begin{figure}[t]
	\begin{tabular}{l c r}
		\begin{subfigure}[t]{0.3\textwidth}
			\scalebox{1}{\usebox{\figownrpd}}
			\caption{Pure-Dataflow (PD)}
			\label{fig:own-reduced-PD}
		\end{subfigure}
		%\hspace{-10pt}
		\begin{subfigure}[t]{0.45\textwidth}
			\raisebox{1.7cm}{\scalebox{0.7}{\usebox{\figownformula}}}
			\caption{\smtlib}
			\label{fig:own-vc-code}
		\end{subfigure}
		%\hspace{50pt}
		\begin{subfigure}[t]{0.20\textwidth}
			\scalebox{1}{\usebox{\figborrpd}}
			\caption{Operations on $\val$ and $\ret{val}$ fat slots for program in~\cref{fig:own-reduced-PD}.}
			\label{fig:bor-reduced-PD}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{Program from~\cref{fig:own-example-C} in PD and \smtlib forms. New ownership intrinsics and their corresponding additions to \smt are highlighted in \marktext{yellow}. Note that the \smt program does not contain $\mathit{write}$ and $\mathit{read}$ expressions. Also note the use of $\boldsymbol{\mathit{z}}$ in borrow and die operations in~\cref{fig:own-reduced-PD}.}
	\label{fig:own-code-vc-translate}
	%\vspace{-0.3in}
\end{figure}

\begin{figure}
	\centering
	\begin{align*}
		\mathit{\entangle}(r_{1},r_{2}) \sdef  & r_{1} = \exists x \cdot x \land r_{2} = r_{1} \text{ where } r_{1},r_{2} \colon \scalar
		\\
		\copyallocinfo(p_{1}, p_{0}) \sdef     & p_{1}.\base = p_{1}.\base \land p_{1}.\off = p_{0}.\off \land p_{1}.\sz = p_{0}.\sz     \\
		                                       & \text{ where } p_{0},p_{1} \colon \ptrsort                                              \\
		\copyoffsetinfo(p_{1}, p_{0}, r) \sdef & p_{1}.\base = p_{1}.\base \land p_{1}.\off = p_{0}.\off + r \land p_{1}.\sz = p_{0}.\sz \\
		                                       & \text{ where } p_{0},p_{1} \colon \ptrsort \text{ and } r \colon \scalar                \\
		\copyvalinfo(p_{1}, p_{0}) \sdef       & p_{1}.\val = p_{0}.\val \land p_{1}.\ret{\val} = p_{0}.\ret{\val}
		\text{ where } p_{0},p_{1} \colon \ptrsort                                                                                       \\
		\mathit{\freshenval}(p) \sdef          & \exists x,y \cdot p.\val = x \land{} p.\ret{val} = y \text{ where } p \colon \ptrsort
	\end{align*}
	\caption[Helper specifictions.]{Helper specifications for Ownership semantics.}
	\label{fig:own_sem_helpers}
\end{figure}

\begin{figure}
	\centering
	\begin{align*}
		\symsub{1}{\tcode{o = mk\_own p}} \sdef         &
		\copyallocinfo(o, p) \land \freshenval(o)                                                                      \\
		% set and get prop
		\symsub{1}{\tcode{p1 = set\_prop p0,\ v}} \sdef &
		\copyallocinfo(p_{1}, p_{0}) \land p_{1}.\val = v                                                              \\
		\symsub{1}{\tcode{r = get\_prop p}} \sdef       & v = p.\val                                                   \\
		\symsub{1}{\tcode{u = begin\_unique p}} \sdef   &
		\symsub{1}{\tcode{u = mk\_own p}}                                                                              \\
		\symsub{1}{\tcode{p = end\_unique u}} \sdef     & \symsub{1}{\tcode{u = mk\_own p}}                            \\ \\
		                                                & \textit{ where } o,u,p_{i} \colon \ptrsort, v \colon \scalar
	\end{align*}
	\caption[Own Creation Semantics (v1)]{Specifications for Ownership creation semantics (version 1)}
	\label{fig:own_sem_create_v1}
\end{figure}


\bparagraph{Creation and properties.}
% Conventionally, for example in \rust, owning pointers are responsible for de-allocation of memory.
% %Thus a pointer created using a \code{malloc} or \code{alloca} is implicitly owning.
% For this presentation, we do not target temporal memory safety (use-after-free, double-free etc.) specifically and instead ownership as stand-in for uniqueness\footnote{We differentiate between Owning pointers and borrowed pointers for some operations. This is discussed more in~\cref{sec:safety}.}.
An \ownptr is created using the \code{mk_own} operation.
The semantics of \code{mk_own} are given in~\cref{fig:own_sem_create_v1}.
The operation consumes a pointer (arguably one that is freshly created using  \code{malloc} or \code{alloca}) and creates a new pointer with the same allocation information except that the $\val$ and $\ret{val}$ fat slots have fresh non-deterministic values.
The \code{set_prop} operation sets the $\val$ slot of a pointer and \code{get_prop} operation gets the value.

To give an intuition of the VCGen process for \code{mk_own} and \code{set_prop}, we take example~\cref{fig:example-C} and add ownership semantics to it in~\cref{fig:own-example-C}.
The corresponding \oseair program is in~\cref{fig:own-reduced-PD} and the \smt program in~\cref{fig:own-vc-code}.
We assume that the \voi is the 1-byte data stored through pointer \code{p}.
The \code{SEA_MKOWN} in~\cref{fig:own-example-C},~\cref{line:own-example-C-mkown} creates an \code{mk_own} instruction in the \oseair program in~\cref{fig:own-reduced-PD}.
The \code{mk_own} instruction in-turn generates \smt semantics as shown in~\cref{fig:own-vc-code}.

To support gradual development of ownership semantics in programs that do not already contain these concepts, pointers can be marked as being unique within a code region and assumed to have aliases outside this scope.
The \code{begin_unique} and \code{end_unique} operations mark the start and end scope where a pointer is unique.
The semantics for this category is given in~\cref{fig:own_sem_create_v1}.
$sym_{1}$ denotes the translation function that encodes an \oseair
program into a VC.
\begin{figure}
	\centering
	\begin{align*}
		% borrow semantics
		\symsub{1}{\tcode{b = mut\_mkbor p},\ \tcode{s = mut\_mksuc p}} \sdef        &
		\copyallocinfo(s, p) \land
		\copyallocinfo(b, p) \land                                                                                                            \\
		                                                                             & \entangle(b.\ret{\val}, s.\val) \land
		s.\ret{\val} = p.\ret{\val} \land                                                                                                     \\
		                                                                             & b.\val = p.\val                                        \\
		\symsub{1}{\tcode{b = mut\_mkbor\_off p r},\ \tcode{b = mut\_mksuc p}} \sdef &
		\copyallocinfo(s, p) \land
		\copyoffsetinfo(b, p, r) \land                                                                                                        \\
		                                                                             & \entangle(b.\ret{\val}, s.\val) \land
		s.\ret{\val} = p.\ret{\val} \land                                                                                                     \\
		                                                                             & b.\val = p.\val                                        \\
		% die
		\symsub{1}{\tcode{die p}} \sdef                                              & p.\val = p.\ret{val}                                   \\ \\
		                                                                             & \text{ where } p,s,b \colon \ptrsort, r \colon \scalar
	\end{align*}
	\caption[Own Semantics (v1)]{Specifications for Mutable borrow Semantics (version 1)}
	\label{fig:own_sem_borrow_v1}
\end{figure}

\bparagraph{Mutable Borrow and Die.}
A mutable borrow operation creates a \mutborptr and a \sucptr.
In a valid program, the \sucptr gets read-write access only after the \mutborptr has completed all reads and writes through it (i.e., has \emph{died}).
A program explicitly marks death of a pointer using a \code{die} operation.
Note that this scheme disallows interleaved accesses between the \mutborptr and \sucptr.

There is no overlap in operations through the \mutborptr and \sucptr.
This allows us to carry a \voi at each alias and transfer the \voi when the alias dies.
% To facilitate the transfer back from borrower to successor we use a prophecy (non-deterministic) \voi that is injected into the successor during a borrow operation but is only materialized when the borrow ends to be equal to the \voi stored in the borrowing pointer.
%The end of borrow is explicitly signalled using a \code{die} operation on the \mutborptr.

% In \oseair, the mutable borrow operation is split into two intrinsics that always occur together in a program.
% The first, \mutborbor creates the \mutborptr and the second, \mutborsuc creates the \sucptr.
The transfer of \voi from \ownptr to \mutborptr occurs through a \mutborbor operation.
The transfer back from \mutborptr to \sucptr occurs through a prophecy variable.
To explain the use of prophecy variables in maintaining a \voi across borrows, see ~\cref{fig:bor-reduced-PD}.
This is a simplified representation of~\cref{fig:own-reduced-PD} and draws out the \smt expressions generated at key steps in the program.
Specifically, \mutborbor and \mutborsuc create $\mathit{p_{5}}$, the \mutborptr, and $\mathit{p_{6}}$, the \sucptr, respectively.
The \val fat slot of $\mathit{p_{6}}$ is \emph{entangled} with the \ret{val} fat slot of $\mathit{p_{5}}$.
The prophecy variable is denoted by $\mathit{z}$.
On a \code{die} operation, the \mutborptr returns the \voi in its $\val$ slot to the \sucptr by setting $\mathit{p_{24}}.\ret{val}=\mathit{p_{24}}.\val$.
The detailed semantics of \mutborbor and \mutborsuc intrinsics is given in~\cref{fig:own_sem_borrow_v1}.

\bparagraph{Read only Borrow and Copy.}
A read only borrow operation creates a \roborptr and a \sucptr.
Both pointers have interleaved, but read only, access until the \roborptr dies.
After this, the \sucptr gets read-write access.
The \voi can be maintained across aliases since each alias is read-only and thus does not mutate the \voi.
A copy operation creates two copying pointers\footnote{These are called raw pointers in \rust.}.
Each \cpyptr has read write access.
A \voi cannot be maintained across copying operations since there are multiple pointers with write access and the \voi may be changed through any pointer.
The semantics of read only borrow and copy operations are given in~\cref{fig:own_sem_bor_ro_cp_v1}.

\begin{figure}
	\centering
	\begin{align*}
		% borrow ro semantics
		\symsub{1}{\tcode{b = robor\_mkbor p},\ \tcode{s = robor\_mksuc p}} \sdef            &
		\copyallocinfo(s, p) \land
		\copyallocinfo(b, p) \land                                                                                                                          \\
		                                                                                     & \copyvalinfo(s, p) \land
		\copyvalinfo(b, p)                                                                                                                                  \\
		% borrow ro w offset
		\symsub{1}{\tcode{b = robor\_mkbor\_off p,\ r},\ \tcode{s = bor\_mksuc\_ro p}} \sdef &
		\copyallocinfo(s, p) \land
		\copyoffsetinfo(b, p, r) \land                                                                                                                      \\
		                                                                                     & \copyvalinfo(s, p) \land
		\copyvalinfo(b, p)                                                                                                                                  \\
		% copy semantics
		\symsub{1}{\tcode{c1 = cpy\_mkcpy1 p},\ \tcode{c2 = cpy\_mkcpy2 p}} \sdef            &
		\copyallocinfo(c_{1}, p) \land
		\copyallocinfo(c_{2}, p) \land                                                                                                                      \\
		                                                                                     & \freshenval(c_{1}) \land \freshenval(c_{2})                  \\
		% copy semantics w offset
		\symsub{1}{\tcode{c1 = cpy\_mkcpy1\_off p,\ r},\ \tcode{c2 = cpy\_mkcpy2 p}} \sdef   &
		\copyallocinfo(c_{2}, p) \land
		\copyoffsetinfo(c_{1}, p, r) \land                                                                                                                  \\
		                                                                                     & \freshenval(c_{1}) \land \freshenval(c_{2})                  \\ \\
		                                                                                     & \text{ where } c_{i},p,b,s \colon \ptrsort, r \colon \scalar
	\end{align*}
	\caption[Own Semantics (v1)]{Specifications for Borrow Read-Only and Copy Semantics (version 1)}
	\label{fig:own_sem_bor_ro_cp_v1}
\end{figure}

\begin{figure}
	\centering
	\begin{align*}
		% bor_mem2reg
		\symsub{1}{\tcode{b,\ m1 = bor\_mem2reg pp,\ m0}} \sdef &
		p = \mathit{read}(m_{0}, pp) \land{}
		\copyallocinfo(s, p) \land                                                                                               \\
		                                                        & \copyallocinfo(b, p) \land
		\entangle(b.\ret{\val}, s.\val) \land                                                                                    \\
		                                                        & s.\ret{\val} = p.\ret{\val} \land
		b.\val = p.\val \land{}                                                                                                  \\
		                                                        & m_{1}= \mathit{write}(m_{0}, s, pp)                            \\
		% mv_reg2mem semantics
		\symsub{1}{\tcode{m1 = mov\_reg2mem p,\ pp,\ m0}} \sdef &
		m_{1} = \mathit{write}(m_{0}, p, pp) \land{} \symsub{1}{\tcode{die p}}                                                   \\ \\
		                                                        & \text{ where } pp,p,b,s \colon \ptrsort, m_{i} \colon \memsort
	\end{align*}
	\caption[Own Semantics (v1)]{Specifications for Borrowing and Moving between registers and memory (version 1).}
	\label{fig:own_sem_read_write_v1}
\end{figure}

\bparagraph{Register--Memory transfer.}
Programs may need to store and load pointers from memory.
In ownership semantics, this is accomplished in the following way.
The intrinsic \movregtomem moves an \ownptr with all fat slots into memory.
Thus, there can be no further actions on the \ownptr.
A pointer that has been moved into memory may be borrowed (with all fat slots) to a register for operations using the \mutbormemtoreg operation.
The semantics for these operations are given in~\cref{fig:own_sem_read_write_v1}.

\subsection{Whole program analysis.}

\newsavebox{\figunsafeexample}
\begin{lrbox}{\figunsafeexample}%
	\begin{lstlisting}[language=C]
extern void escapeToMemory(char *);
int main() {
  char *p = (char *)malloc(sizeof(char));
  *@\marktext{SEA\_MKOWN(p);}@* *@\label{line:own-example-C-mkown} @*
  char c = nd_char();
  assume (c == 0);
  *@\marktext{SEA\_SET\_PROP(p, c);}@* *@\label{line:unsafe-example-C-setprop} @*
  *p = c;
  char *cp1;
  *@\marktext{SEA\_COPY(cp1, p);}@* *@\label{line:unsafe-example-C-copy} @*
  if (nd_bool()) {
    c = nd_char();
    assume(c > 1);
    *cp1 = c;
    escapeToMemory(cp1);
    c = *cp1;
  }
  *@\marktext{SEA\_DIE(cp1);}@*
  *@\marktext{SEA\_SET\_PROP(p, c);}@*  *@\label{line:unsafe-example-C-reload} @*
  char r;
  *@\marktext{SEA\_GET\_PROP(p, r);}@*
  sassert(r == 0 || r > 1);
  *@\marktext{SEA\_DIE(p);}@*
  return 0;
}
\end{lstlisting}%
	%\vspace{-0.3in}
\end{lrbox}%


\newsavebox{\figunsaferpd}
\begin{lrbox}{\figunsaferpd}%
	\begin{lstlisting}
fun main() {
BB0:
  M3 = mem.init()
  P0, M0 = malloc 1, M3
  *@\marktext{P2 = mk\_own P0}@*
  R5 = nd_char()
  R6 = R5 == 0
  *@\marktext{p3 = set\_prop P2 R5}@*
  M1 = store R5, P3, M0
  *@\marktext{P5 = cpy\_mkcpy1 P3}@*
  *@\marktext{P6 = cpy\_mkcpy2 P3}@*
  R15 = nd_bool();
  R17 = R15 == 0
  br R17, ERR, BB1

BB1:
  R28 = nd_char()
  R29 = R28 > 1
  R30 = R6 && R29
  *@\marktext[blue!30]{M2 = store R28, P5, M1}@*
  escapeToMemory(P5)
  *@\marktext[blue!30]{R35 = load P5, M2}@*
  br ERR

ERR:
  R38 = select R17, R6, R30
  R39 = select R17, R5, R35
  *@\marktext{die P5}@*
  *@\marktext{P10 = set\_prop P6 R39}@*
  *@\marktext{R42 = get\_prop P10}@*
  R44 = R42 == 0
  R45 = R42 > 1
  R46 = R44 || R45
  A = not R46
  assume A
  assert false
  halt
}
\end{lstlisting}
\end{lrbox}%

\newsavebox{\figunsafeformula}
\begin{lrbox}{\figunsafeformula}%
	$
		\begin{array}{l}
			\sind[1] p_{0}.\base = \mathit{addr}_{0} \land{} p_{0}.\off = 0 \land{} p_{0}.\sz = 1 \land{}    \\
			\sind[1] \marktext{$p_{2} = \copyallocinfo(p_{2}, p_{0}) \land{} \freshenval(p_{2})$} \land{}    \\
			\sind[1] r_{6} = (r_{5} = 0) \land{}                                                             \\
			\sind[1]\marktext{$ \copyallocinfo(p_{3}, p_{2}) \land{} p_{3}.\val = r_{5}$}  \land{}           \\
			\sind[1] \marktext{$\copyallocinfo(p_{5}, p_{3}) \land{} \copyallocinfo(p_{6}, p_{3}) \land{} $} \\
			\sind[1] \marktext{$\freshenval(p_5) \land{} \freshenval(p_6) \land{} p_{5}.\val$} \land{}       \\
			\sind[1] r_{17} = (r_{15} = 0) \land{}                                                           \\
			\sind[1] r_{29} = r_{28} > 1 \land{}                                                             \\
			\sind[1] r_{30} = r_{6} \land{} r_{29} \land{}                                                   \\
			\sind[1] \marktext[blue!30]{$m_2=write(m_1,p_{5})$} \land{}                                      \\
			\sind[1] \marktext[blue!30]{$r_{35} = read(m_2,p_{5}) $} \land{}                                 \\
			\sind[1] r_{38}=ite(r_{17}, r_{6}, p_{30}) \land{}                                               \\
			\sind[1] r_{39}=ite(r_{17}, r_{5}, r_{35}) \land{}                                               \\
			\sind[1] \marktext{$p_{5}.\ret{val} = p_{5}.\val$} \land{} r_{38} \land{}                        \\
			\sind[1] \marktext{$\copyallocinfo(p_{10},p_6) \land{} p_{10}.\val=r_{39}$} \land{}              \\
			\sind[1] \marktext{$r_{42} = p_{10}.\val$} \land{}                                               \\
			\sind[1] r_{44} = r_{42} = 0 \land{}                                                             \\
			\sind[1] r_{45} = r_{42} > 1 \land{}                                                             \\
			\sind[1] r_{46} = (r_{44} \lor r_{45}) \land{}                                                   \\
			\sind[1] a = \neg r_{46} \land{}                                                                 \\
			\sind[1] a \land{}                                                                               \\
			\sind[1] \neg \mathit{false}
		\end{array}
	$
\end{lrbox}%

\begin{figure}[t]
	\begin{tabular}{l c r}
		\begin{subfigure}[t]{0.4\textwidth}
			\scalebox{1}{\usebox{\figunsafeexample}}
			\caption{C program.}
			\label{fig:unsafe-example-C}
		\end{subfigure}
		\begin{subfigure}[t]{0.3\textwidth}
			\scalebox{1}{\usebox{\figunsaferpd}}
			\caption{Pure-Dataflow (PD)}
			\label{fig:unsafe-reduced-PD}
		\end{subfigure}
		%\hspace{-10pt}
		\begin{subfigure}[t]{0.4\textwidth}
			\raisebox{1.7cm}{\scalebox{0.7}{\usebox{\figunsafeformula}}}
			\caption{\smtlib}
			\label{fig:unsafe-vc-code}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{C program with owned and copy operations in PD and \smtlib forms. Ownership intrinsics and \smt counterparts are highlighted in \marktext{yellow}.  Note that the \smt program contains $\mathit{write}$ and $\mathit{read}$ expressions through \cpyptr $p_{5}$ in \marktext[blue!30]{blue}.}
	\label{fig:unsafe-code-vc-translate}
	%\vspace{-0.3in}
\end{figure}

To study the effect of copy operations on a program with ownership semantics.
We modify our running C example by replacing the borrow with a copy operation in~\cref{fig:unsafe-example-C},~\cref{line:unsafe-example-C-copy}.
A write and read through a \cpyptr must go to memory since multiple mutable aliases may operate in an interleaved manner.
Thus memory accesses need to be modeled for such a pointer.
However, the rest of the program can operate as before, using ownership semantics.
For this, once the copy \code{cp1} dies, the \ownptr \code{p} reloads the property from memory at~\cref{line:unsafe-example-C-reload} and further accesses through \code{p} do not result in memory accesses.
Thus a single write-read expression exists in~\cref{fig:unsafe-vc-code}.


==> properties.tex <==
\section{Carrying Properties with Fat Pointers.}
\label{sec:prop}

So far, we have not discussed what a \voi may be.
From the discussion so far, we show it to be a \scalar type.
We now present the reasoning behind this decision and discuss properties that a \voi may represent.

We present various design choices for data that can be carried at a pointer:
\begin{enumerate}
\item All bits (of an allocation) that a pointer can directly access may be carried at a pointer.
However, this is expensive since for efficiency memory is modelled more abstractly (e.g., as a lambda abstraction) and translating between a low-level representation and memory abstraction during synchronization is expensive.
\item We can instead carry an abstract memory representation of an allocation. This would be computationally cheap during synchronization.
        However, it introduces a problem that
        when the value of a prophecy variable is constrained (on a \code{die}), it results in an equality.
        This equality over lambda abstractions can be computationally expensive to ascertain,
        requiring enumerating equality over all possible values (i.e., extensional theory of arrays) and we want to avoid bringing in this machinery into our solving pipeline.
\end{enumerate}
A solution is to carry \scalar values that represent object typestates~\cite{DBLP:journals/tse/StromY86}.
As types determine the set of valid operations on an object, typestates determine the set of valid operations on an object in a context.
Capturing and tracking typestates also maps well to \bmc where such properties represent precise operations on data in a lightweight (and hence scalable) manner.
We present some properties that a \voi can represent and hence can be carried at pointers.
\begin{enumerate}
  \item Primitive typestate properties. For example, number of times \code{encrypt_buf} has been called on some buffer.
  \item Sequence typestate properties. For example in a SSL/TCP library, a successful send must call 1) encrypt, 2) send, and 3) clear send buffer in that order.
  \item Predicate typestate properties. For example, testing that \code{memset} is always called with length parameter that is equal to the length of allocation.
\end{enumerate}

All these flavours of typestate properties have a characteristics that their state can be expressed as \scalar.
We will discuss our findings on what can be interesting \voi as the evaluation in~\cref{sec:ownsem-eval} proceeds.


==> proposal.tex <==
\section{Background and Problem Def}
\label{sec:intro}

% \sid{
% We present the work in three steps.
% \begin{itemize}
%   \item [Motivation] Where are we coming from -- whole program verification in a low level language with both safe and unsafe accesses -- and why is this space interesting for ownership semantics
%   \item [Problem Definition] The problems in mapping RustHorn semantics to this setting: How to model replacing refs-to-values by values. Also what are values?
%   \item [Contributions] \dots
% \end{itemize}
% By using this breakup, the hope is to tweak each part independently of the other.
% }

% \begin{enumerate}
%   \item Using uniqueness/ownership for program verification has been used in RustHorn before in a high level setting.
%   \item In a low-level setting, both safe and unsafe accesses exist.

% 1. Scalable BMC is dependent on efficient VCGen from source program.
% 1. Using a simple IR (like SEA-IR) is a good starting point to study VCGen [see previous work for motivation]
% 1. SEA-IR models concepts from source language + its own analysis
% 1. However, it lacks ownership of resources (resource is a chunk of memory as opposed to a scalar value) that Rust programs carry.
% 1. We show how adding this information results in simpler VCs.
%\end{enumerate}                 %
%\sid{START: setup problem space}

% In \rust, the programmer communicates aliasing restrictions on references using concepts of ownership and borrowing.
% References that are owned, subsequently mutably borrowed and then returned remain unique during these series of operations.
% For program verification, if a reference follows ownership and borrowing discipline then the reference can be replaced by the value it refers to.
% This was exploited in the RustHorn work which uses prophecy variables to model the future value of reference after a borrow ends.
% More generally though, in programs, some operations use unique reference to objects while other operations require multiple references (e.g., graph node with multiple edges).
% The former thus fits into the safe borrowing discipline of \rust while the latter is expressed using the \code{unsafe} keyword in \rust.
% Thus, in the presence of \code{unsafe} operations, we cannot get away from modelling memory for verification.
% Our insight is that in the context of automatic program verification of programs with ownership semantics,
% we need not be compelled to choose between verifying only safe programs or back each reference with a memory model for unsafe programs.
% Thus
% \begin{enumerate}
%   \item We can replace owned (or borrowed) references with values [shown in move prover/RustHorn], and
%   \item we can apply prophecy variables to model the return value of a borrow [RustHorn], and
%   \item only when multiple references to an object exist, do we model the memory behind the object [our insight]
% \end{enumerate}

Formal verification of programs with low-level control like C/C++ and \rust usually requires modelling memory since programs explicitly operate on memory.
\rust, specifically, adds uniqueness and linear guarantees to data (and references) using owned and borrowed concepts.
However, these guarantees are only available in \emph{safe} \rust.
Unsafe \rust code, allows aliasing and cannot be proved safe by the \rust compiler.

The RustHorn verification paper showed that one can precisely verify properties of programs in a safe subset of Rust without modelling memory.
The key insight there is to replace unique references with values and to use prophecy variables to model borrows.

While the verification of safe Rust can do away with modelling memory,
it has been shown empirically that practical \rust programs are not usually bound to a safe subset of \rust but use unsafe semantics that allows for more general and unconstrained computation.
For example, this is the case for graph data structures where verification must assume multiple aliases to refer to the same node.
This work studies how ideas from RustHorn -- references as values and prophecy variables can be utilized to whole program automatic verification that has access patterns in both owned and aliased settings.

We specifically choose to use \seair (\llvm IR) language to conduct this work.
\seair is symbolically executed on the \seabmc engine which is a bit-precise bounded model checking engine for \seahorn.
\seair offers a low level and uniform view of different memory access patterns and the advantages of \llvm IR for VCGen has been studied previously.
In \llvm IR, references of higher level languages map to pointers.
Mapping of higher level values is dealt with later in this article.
We now consider two main technical challenges in applying the learnings of RustHorn in our setting.
\begin{enumerate}
  \item We want to opportunistically do away with modelling memory for owned operations but model it faithfully in the presence of aliasing. How can we signal to the VCGen process when to model memory and when to not, i.e. to do so lazily?
  \item What is equivalent to a value prophesized in RustHorn{,Belt} for \seair?
  %\item Customary 3rd point
\end{enumerate}
We now elaborate on these challenges.

\bparagraph{To model or not to model (memory)?}
We want our lazy memory model to have the following properties.
\begin{enumerate}
  \item Avoid memory look ups when pointers are known to be unique and somehow carry the pointed-to value outside of memory as the program executes.
  \item At the same time, model load, store instructions and underlying memory faithfully in the presence of aliasing.
  \item Lastly, have an ability to synchronize between the carried value and the value in memory such that the program with a lazy memory model is equivalent to one with an eager memory model.
\end{enumerate}

In the \seabmc setting, we already model memory in a bit-precise manner and carry allocation info in fat-pointers.
We now utilize fat-pointers to carry arbitrary program values, including prophesized values, in their fat slots.
We also introduce new intrinsics in \seair that create new pointer types -- owned, borrowed
and signal when values between memory and pointers need to be synced.
This creates a symex machine with both underlying memory and fat-pointers that can store out-of-memory values and most importantly an ability to synchronize between memory and fat-pointers in the presence of aliasing.
To evaluate our programming environment, we compile programs written in C to our machine.
Since C does not have ownership semantics, we augment C with MACROS that the programmer uses to specify ownership constraints on pointers.

So far, we have let the problem of what a value is remain amorphous.
We now give it some shape.

\bparagraph{What is a \emph{value}?}
By using prophecy variables and eliminating the need to model memory,
RustHorn is able represent program values in pure FOL.
In the setting of \seabmc, all values are bitvectors and pointers map locations to values.
Thus what values do we carry outside of memory?
We present some options and their shortcomings:
\begin{enumerate}
\item We can carry all the bits (of an allocation) that a pointer can directly access.
However, this is expensive since for efficiency memory is modelled more abstractly (as a lambda abstraction) and translating between a reified value and memory during synchronization is expensive.
\item We can instead carry an abstract memory representation of an allocation. This would be computationally cheap during synchronization.
        However, it introduces a problem that
        when the value of a prophecy variable is materialized, it results in an equality.
        This equality over lambda abstractions can be computationally expensive to ascertain,
        requiring enumerating equality over all possible values (i.e., extensional theory of arrays) and we want to avoid bringing in this machinery into our solving pipeline.
\end{enumerate}
% We proceed towards a solution by recognizing two characteristics:
% First, \CaS and \bmc favour
% crafting correctness proofs to be property checks on scalars.
% These scalars may summarize a property of aggregate data.
% For example, see how \awsccommon \cas proofs check that two buffers are byte-by-byte equivalent --
% by recording a non-deterministic index in a ghost variable and comparing bytes in both buffers at the same index.
% This is in contrast how one would naively expect to compare bytes -- iterate over the whole buffer and compare each byte.
% Or, see how \verifyccommon proofs for \seabmc use \code{is_mod} to check that a buffer is unmodified.
% We set a bit whenever a write occurs and check its value rather than recording the whole buffer and checking it byte-by-byte to check immutation.
We proceed towards a solution by recognizing that \CaS and \bmc often times favours checking properties of program state by asserting that side-state (or typestate) properties hold.
\begin{enumerate}
  \item Primitive typestate properties. For example, number of times \code{encrypt_buf} has been called on some buffer.
  \item Sequence typestate properties. For example in a SSL/TCP library, a successful send must call 1) encrypt, 2) send, and 3) clear send buffer in that order.
  \item Predicate typestate properties. For example, testing that \code{memset} is always called with length parameter that is equal to the length of allocation.
\end{enumerate}

All these flavours of typestate properties have a characteristics that their state can be expressed as a scalar.
Now this scalar can be carried by fat pointers.
We call such typestate carrying fat pointers \emph{Carrier Pointers}.\sid{nee. lazy pointers, proof carrying pointers, summary pointers, sidestate pointers, typestate pointers}.

introduction
background


==> safety.tex <==
\section{Checking Ownership Semantics.}
\label{sec:safety}

\newsavebox{\figbortakesloan}
\begin{lrbox}{\figbortakesloan}%
	\centering
	\begin{forest}
		for tree={
		draw,
		minimum height=2cm,
		anchor=north,
		align=center,
		child anchor=north
		},
		[{P\\\begin{tabular}{|c|c|c|c|c}
							\hline
							$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
							\hline
							$p$            & 1             & $l_{p}$         & \marktext[pink!60]{$l_{a}$} & ... \\
							\hline
						\end{tabular}}
					[{S\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$ & ... \\
									\hline
									$s$            & 1             & $0$         & $0$         & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,left] {\mutborsuc}}
					]
					[{B\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
									\hline
									$b$            & $1+l_{a}$     & $0$         & \marktext[pink!60]{$l_{a}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,right] {\mutborbor}}
					]
			]
	\end{forest}
\end{lrbox}

\newsavebox{\figsuctakesloan}
\begin{lrbox}{\figsuctakesloan}%
	\centering
	\begin{forest}
		for tree={
		draw,
		minimum height=2cm,
		anchor=north,
		align=center,
		child anchor=north
		},
		[{P\\\begin{tabular}{|c|c|c|c|c}
							\hline
							$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$    & $\mathit{held}$             & ... \\
							\hline
							$p$            & 1             & $l_{p}$ & \marktext[pink!60]{$l_{a}$} & ... \\
							\hline
						\end{tabular}}
					[{S\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$             & ... \\
									\hline
									$s$            & $1+l_{s}$     & \marktext{$l_{s}$}         & \marktext[pink!60]{$l_{a}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,left] {\mutborsuc}}
					]
					[{B\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
									\hline
									$b$            & $1+l_{s}$     & $0$         & \marktext{$l_{s}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,right] {\mutborbor}}
					]
			]
	\end{forest}
\end{lrbox}

\newsavebox{\figtreemutbor}
\begin{lrbox}{\figtreemutbor}%
	\centering
	\begin{forest}
		for tree={
		draw,
		minimum height=2em,
		anchor=north,
		align=center,
		child anchor=north
		},
		[,coordinate
		[{PA\\\begin{tabular}{|c|c|c|c|c}
					\hline
					$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$    & $\mathit{held}$ & ... \\
					\hline
					$p_{a}$        & 1             & \marktext[pink!60]{$l_{a}$} & $h_{p_{a}}$     & ... \\
					\hline
				\end{tabular}}, align=center, name=PA
		[{SA\\\begin{tabular}{|c|c|c|c|c}
					\hline
					$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$ & ... \\
					\hline
					$s_{a}$        & $1+l_{a}$     & $0$     & $h_{p_{a}}$     & ... \\
					\hline
				\end{tabular}},edge label={node[midway,left]{\mutborbor}}, name=SA
		]
		[{BA}, edge label={node[midway,right]{\mutborbor}}, name=BA
		[,phantom] % Adjust for alignment
		[{P},edge=dashed, name=P
		[{S},edge label={node[midway,left]{\mutborsuc}}, name=S]
		[{B\\\begin{tabular}{|c|c|c|c|c}
					\hline
					$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
					\hline
					$b$            & $1+l_{a}$     & $0$         & \marktext[pink!60]{$l_{a}$} & ... \\
					\hline
				\end{tabular}}, edge label={node[midway,right]{\mutborbor}}, name=B]
		]
		]
		]]
	\end{forest}
\end{lrbox}

% Begin copy scheme
\newsavebox{\figowngivesloan}
\begin{lrbox}{\figowngivesloan}%
	\centering
	\begin{forest}
		for tree={
		draw,
		minimum height=2cm,
		anchor=north,
		align=center,
		child anchor=north
		},
		[{P\\\begin{tabular}{|c|c|c|c|c}
							\hline
							$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
							\hline
							$p$            & 1             & $l_{p}$         & \marktext{$h_{p}$} & ... \\
							\hline
						\end{tabular}}
					[{S\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$ & ... \\
									\hline
									$s$            & 1             & $l_{s}$         & $h_{s}$         & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,left] {\cpyone}}
					]
					[{C\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
									\hline
									$c$            & $1+h_{p}$     & $l_{c}$         & \marktext{$h_{p}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,right] {\cpytwo}}
					]
			]
	\end{forest}
\end{lrbox}

\newsavebox{\figcpysuckeepsloan}
\begin{lrbox}{\figcpysuckeepsloan}%
	\centering
	\begin{forest}
		for tree={
		draw,
		minimum height=2cm,
		anchor=north,
		align=center,
		child anchor=north
		},
		[{P\\\begin{tabular}{|c|c|c|c|c}
							\hline
							$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$    & $\mathit{held}$             & ... \\
							\hline
							$p$            & 1             & \marktext{$l_{p}$} & \marktext[pink!60]{$h_{p}$} & ... \\
							\hline
						\end{tabular}}
					[{S\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$             & ... \\
									\hline
									$s$            & $1+l_{p}$     & $l_{s}$         & \marktext[pink!60]{$h_{p}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,left] {\cpyone}}
					]
					[{C\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
									\hline
									$c$            & $1+l_{p}$     & $l_{c}$         & \marktext{$l_{p}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,right] {\cpytwo}}
					]
			]
	\end{forest}
\end{lrbox}

\newsavebox{\figcpyonetakesloan}
\begin{lrbox}{\figcpyonetakesloan}%
	\centering
	\begin{forest}
		for tree={
		draw,
		minimum height=2cm,
		anchor=north,
		align=center,
		child anchor=north
		},
		[{C\\\begin{tabular}{|c|c|c|c|c}
							\hline
							$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
							\hline
							$c$            & $rc_{c}$      & $l_{c}$         & \marktext{$h_{c}$} & ... \\
							\hline
						\end{tabular}}
					[{C1\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$ & ... \\
									\hline
									$c_{1}$        & $rc_{c_{1}}$  & $l_{c_{1}}$     & $h_{c_{1}}$     & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,left] {\cpyone}}
					]
					[{C2\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
									\hline
									$c_{2}$        & $rc_{c_{2}}$  & $l_{c_{2}}$     & \marktext{$h_{c}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,right] {\cpytwo}}
					]
			]
	\end{forest}
\end{lrbox}

\newsavebox{\figcpytwotakesloan}
\begin{lrbox}{\figcpytwotakesloan}%
	\centering
	\begin{forest}
		for tree={
		draw,
		minimum height=2cm,
		anchor=north,
		align=center,
		child anchor=north
		},
		[{C\\\begin{tabular}{|c|c|c|c|c}
							\hline
							$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
							\hline
							$c$            & 1             & $l_{c}$         & \marktext{$h_{c}$} & ... \\
							\hline
						\end{tabular}}
					[{C1\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$    & ... \\
									\hline
									$c_{1}$        & $rc_{c_{1}}$  & $l_{rc_{1}}$    & \marktext{$h_{c}$} & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,left] {\cpyone}}
					]
					[{C2\\\begin{tabular}{|c|c|c|c|c}
									\hline
									$\mathit{ptr}$ & $\mathit{RC}$ & $\mathit{lent}$ & $\mathit{held}$ & ... \\
									\hline
									$c_{2}$        & $rc_{c_{2}}$  & $l_{c_{2}}$     & $l_{c_{2}}$     & ... \\
									\hline
								\end{tabular}}, edge label={node[midway,right] {\cpytwo}}
					]
			]
	\end{forest}
\end{lrbox}


\begin{figure}[t]
	\begin{subfigure}[t]{0.45\textwidth}
		\scalebox{0.65}{\usebox{\figsuctakesloan}}
		\caption{\Sucptr S lends loan $l_{s}$  to \mutborptr B and holds loan $l_{a}$.}
		\label{fig:suc-takes-loan}
	\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\scalebox{0.65}{\usebox{\figbortakesloan}}
		\caption{P transfers held loan $l_{a}$ to B.}
		\label{fig:bor-takes-loan}
	\end{subfigure}
	\begin{subfigure}[t]{1\textwidth}
		\scalebox{0.65}{\usebox{\figtreemutbor}}
		\caption{Origin of loan $l_{a}$ from~\cref{fig:bor-takes-loan} is from pointer PA.}
		\label{fig:tree-mut-bor}
	\end{subfigure}
	%\hspace{-10pt}
	\caption{Lending scheme during a mutable borrow operation. Two options are possible as shown.}
	\label{fig:safety-bor-check}
\end{figure}

\begin{figure}[t]
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
		\scalebox{0.65}{\usebox{\figcpysuckeepsloan}}
		\caption{\Ownptr (P) lends loan $l_{p}$  to \cpyptr (C) and holds loan $h_{p}$ in \sucptr (S).}
		\label{fig:suc-keeps-loan}
	\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\scalebox{0.65}{\usebox{\figowngivesloan}}
		\caption{P transfers held loan $h_{p}$ to C.}
		\label{fig:own-gives-loan}
	\end{subfigure}
	\\
	\begin{subfigure}[t]{0.45\textwidth}
		\scalebox{0.65}{\usebox{\figcpytwotakesloan}}
		\caption{C transfers held loan $h_{c}$ to \cpyptr (C1).}
		\label{fig:cpy2-takes-loan}
	\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\scalebox{0.65}{\usebox{\figcpyonetakesloan}}
		\caption{C transfers held loan $h_{c}$ to \cpyptr (C2).}
		\label{fig:cpy1-takes-loan}
	\end{subfigure}
	\caption{Lending scheme during a copy operation. An \ownptr as source may lend. However a \cpyptr as source may only transfer held loan to either copies.}
	\label{fig:safety-cpy-check}
\end{figure}

% text begins

In \seair, without ownership semantics, pointers are defined either through an allocation operation (\code{malloc} and \code{alloca}) or through the \code{gep} operation, which creates an alias for a pointer and may add an offset.
Ownership semantics add other aliasing operations with three key properties:
\begin{inparaenum}
	\item aliasing operations consume the operand (source pointer),
	\item aliasing operations always define two pointers -- leading to a binary tree like structure of aliases,
	\item a \code{die} operation that consumes a pointer (alias) without defining any new pointers.
\end{inparaenum}
These properties can be combined with prophecy symbols to model constraints on mutable borrows, read only borrows and copies.
Further, this is useful in proving that an \oseair program has defined behaviour according to ownership semantics.

We motivate our model of ownership semantics by illustrating a mutable borrow operation in~\cref{fig:safety-bor-check}.
We introduce a concept of a \emph{loan} (noun) and define three new fat slots:
\begin{inparaenum}
	\item A loan is a fresh prophecy symbol stored in a $\lend$ fat slot when a fat pointer is defined,
	\item a fat pointer slot $\held$, holds a loan gotten from another pointer, and,
	\item a fat slot $\rc$ that stores the current reference count (of the number of aliases).
\end{inparaenum}
During a mutable borrow operation, the source pointer may \emph{lend} the loan (in $\lend$ slot) to the \mutborptr.
Alternatively, it may \emph{transfer} the loan it holds in the $\held$ slot to the \mutborptr.
In the first case, shown in~\cref{fig:suc-takes-loan} the loan $l_{p}$ is lent from the source pointer (P) to the \mutborptr (B),
The $\rc$ slot for the \sucptr (S) is set to $1 + l_{p}$.
This $\mathit{entangles}$ S and B pointers such that when B's $\held$ slot ($b.held$) is constrained then a read of S's $rc$ slot ($s.rc$) will observe the constraint.
In the second case,
as shown in~\cref{fig:tree-mut-bor}, a loan from PA is held by P through a tree of successive mutable borrow operations.
Now P transfers the held loan to B, as shown in~\cref{fig:bor-takes-loan}, causing $\mathit{entanglement}$ between the \sucptr SA and B.

Each mutable borrow operation chooses between a \emph{lend} and \emph{transfer} non-deterministically.
Thus in each execution a \sucptr and some child \mutborptr are $\mathit{entangled}$.
In a symbolic execution environment, therefore, all valid $\mathit{entanglements}$ occur.

Finally, when \code{die} is called on B then $b.\held$ is equated to zero.
This can be used to model mutable borrow semantics where, for example, B must die before S can be used as an operand.
For this, a program adds a check that $s.rc = 1$ before a \mutborbor operation, which will be true if \die is called on B in all program executions.
This will catch safety violations which would cause an errant \mutborbor operation to define multiple mutable borrows.


\begin{table}[t]
	\centering
	\rowcolors{2}{purple!30}{pink!60}
	\begin{tabular}{|c|c|}
		\hline
		\rowcolor{gray!15}
		Fat slot    & description                                                     \\
		$\trackown$ & Set to 1 to mark pointer as tracked using ownership semantics.  \\
		$\own$      & Set to 1 to mark pointer as an owning pointer.                  \\
		$\rc$       & Reference count: set to 1 to mark pointer as unique.            \\
		$\wok$      & Write ok: set to 1 to mark write allowed through pointer.       \\
		$\rok$      & Read ok: set to 1 to mark read allowed through pointer.         \\
		$\dieok$    & Die ok: set to 1 to mark \code{die} allowed on pointer.         \\
		$\lend$     & Store the loan the pointer can give in an aliasing operation.   \\
		$\held$     & Store the loan gotten from a pointer in  an aliasing operation. \\
		\hline
	\end{tabular}
	\label{tab:own-fat-slots}
	\caption{Fat slots for ownership semantics.}
\end{table}

\begin{table}[t]
	\centering
	\rowcolors{2}{blue!40}{blue!15}
	\begin{tabular}{|c|c|}
		\hline
		\rowcolor{gray!15}
		operation on source ptr $p$ & check                                                             \\
		\mutborbor,\ \mutborsuc     & $p.\trackown=1 \land{} p.\rc=1 \land{} p.\wok=1 \land{} p.\rok=1$ \\
		\roborbor,\ \roborsuc       & $p.\trackown=1 \land{} p.\rok=1$                                  \\
		\cpyone,\ \cpytwo           & $p.\trackown=1 \land{} p.\wok=1 \land{} p.\rok=1$                 \\
		\die                        & $p.\trackown=1 \land{} p.\dieok=1$                                \\
		memory instr                & TBD                                                               \\
		\hline
	\end{tabular}
	\label{tab:own-valid-check}
	\caption{Fat slots for ownership semantics.}
\end{table}


\begin{figure}[t]
	\centering
	\begin{align*}
		\lend(s,b,p,lend_{s},lend_{b}) \sdef              &
		(s.\rc=1+p.\lend) \land{} s.\lend = lend_{s} \land{} s.\held = p.\held \land{}                                                          \\ & (b.\rc=1+p.\lend) \land{} b.\lend=lend_{b} \land{} b.\held=p.\lend \\
		\transfer(s,b,p,lend_{s},lend_{b},held_{s}) \sdef &
		s.\rc=1 \land{} s.\lend = lend_{s} \land{} s.\held = held_{s} \land{}                                                                   \\
		                                                  & (b.\rc=1+p.\held) \land{} b.\lend=lend_{b} \land{} b.\held=p.\held                  \\
		\mkownown(p) \sdef                                & p.\trackown=1 \land{} p.\own=1 \land{} p.\wok=1 \land{} p.\rok=1 \land{} p.\dieok=1 \\
		\mkmutborbor(b) \sdef                             & b.\trackown=1 \land{} b.\own=0 \land{} b.\wok=1 \land{} b.\rok=1 \land{} b.\dieok=1
	\end{align*}
	\caption[Helper specifictions.]{Additional helper macros for ownership semantics.}
	\label{fig:own_sem_safety_helpers}
\end{figure}

\begin{figure}[t]
	\centering
	\begin{align*}
		\symsub{2}{\tcode{o = mk\_own p}} \sdef       &
		\mkownown(p) \land{} \exists l_{p},h_{p} \cdot (p.\lend = l_{p} \land p.\held = h_{p}) \land{}
		\symsub{1}{\tcode{o = mk\_own p}}                                                                                                                           \\
		\symsub{1}{\tcode{u = begin\_unique p}} \sdef & \mkmutborbor(u) \land{} \exists l_{u} \cdot u.\lend=l_{u} \land{} \exists h_{u}\cdot u.\held=h_{u} \land{}
		\symsub{1}{\tcode{u = begin\_unique p}}                                                                                                                     \\
		\symsub{2}{\tcode{p = end\_unique u}} \sdef   & \exists l_{p},h_{p}\cdot(p.\lend=l_{p} \land{} p.\held=h_{p}) \land{} \symsub{1}{\tcode{p = end\_unique u}} \\
		                                              & \textit{ where } o,u,p \colon \ptrsort
	\end{align*}
	\caption[Own Creation Semantics (v1)]{Specifications for Ownership creation semantics (version 2)}
	\label{fig:own_sem_create_v2}
\end{figure}

\begin{figure}[t]
	\centering
	\begin{align*}
		% helpers
		\mklendmutbor(s,b,p,\lend_{s},\lend_{b}) \sdef                               &
		s.\trackown=1 \land{} s.\own=1 \land{} s.\wok=(1-p.\lend) \land{}                                                                     \\ &
		s.\rok=(1-p.\lend) \land{} s.\dieok=(1-p.\lend) \land{}
		\mkmutborbor(b)
		\land{}                                                                                                                               \\&                             \lend(s,b,p,lend_{s},lend_{b}) \\
		\mktransfermutbor(s,b,p,lend_{s},lend_{b},held_{s}) \sdef                    &
		\mkownown(s) \land{} \mkmutborbor(b) \land{} \transfer (s,b,p,lend_{s},lend_{b},held_{s})                                             \\
		% mutborrow semantics
		\symsub{2}{\tcode{b = mut\_mkbor p},\ \tcode{s = mut\_mksuc p}} \sdef        &
		\exists c,lend_{s},lend_{b},held_{s} \cdot ite(c, \mklendmutbor(s,b,p,\lend_{s},\lend_{b}),                                           \\ &
		\mktransfermutbor(s,b,p,lend_{s},lend_{b},held_{s})) \land{}                                                                          \\ &
		\symsub{1}{\tcode{b = mut\_mkbor p},\ \tcode{s = mut\_mksuc p}}                                                                       \\
		\symsub{1}{\tcode{b = mut\_mkbor\_off p r},\ \tcode{b = mut\_mksuc p}} \sdef &
		\exists c,lend_{s},lend_{b},held_{s} \cdot ite(c, \mklendmutbor(s,b,p,\lend_{s},\lend_{b}),                                           \\ &
		\mktransfermutbor(s,b,p,lend_{s},lend_{b},held_{s})) \land{}                                                                          \\&
		\symsub{1}{\tcode{b = mut\_mkbor\_off p r},\ \tcode{b = mut\_mksuc p}}                                                                \\
		% die
		\symsub{1}{\tcode{die p}} \sdef                                              & p.\held=0 \land{} \symsub{1}{\tcode{die p}}            \\
		                                                                             & \text{ where } p,s,b \colon \ptrsort, r \colon \scalar
	\end{align*}
	\caption[Own Semantics (v2)]{Specifications for Mutable borrow Semantics (version 2)}
	\label{fig:own_sem_borrow_v2}
\end{figure}


==> safetyshort.tex <==
\section{Safety Checking.}
\label{sec:safety}

\begin{mdframed}[backgroundcolor=gray!20, linecolor=black, linewidth=1pt, roundcorner=5pt]
This section describes ongoing work.
\end{mdframed}

In~\cref{sec:lang}, we assume that pointers follow ownership semantics.
We expect this will be true when \oseair will represent a \rust program that has passed the borrow checker.
However, we may still want to check at the \oseair level that pointers do follow these semantics and report violations to the user.
To accomplish, we are developing a path sensitive ownership semantics checker.

